Mixture of Decision Trees for Interpretable Machine Learning

This work introduces a novel interpretable machine learning method called Mixture of Decision Trees (MoDT). It constitutes a special case of the Mixture of Experts ensemble architecture, which utilizes a linear model as gating function and decision trees as experts. Our proposed method is ideally suited for problems that cannot be satisfactorily learned by a single decision tree, but which can alternatively be divided into subproblems. Each subproblem can then be learned well from a single decision tree. Therefore, MoDT can be considered as a method that improves performance while maintaining interpretability by making each of its decisions understandable and traceable to humans. Our work is accompanied by a Python implementation, which uses an interpretable gating function, a fast learning algorithm, and a direct interface to fine-tuned interpretable visualization methods. The experiments confirm that the implementation works and, more importantly, show the superiority of our approach compared to single decision trees and random forests of similar complexity.

==> 99-removed.tex <==
\begin{table}[t!]
\caption{Comparison of the gating function variants}
\begin{center}
\begin{tabular}{ |r|r|r||r|r| } 
\hline
dataset & \ac{2D} training & \ac{FG} training & \ac{2D} test & \ac{FG} test \\
\hline

abalone & .74 $\pm$ .00 & .75 $\pm$ .01 & .71 $\pm$ .01 & \cellcolor{custom-grey} .73 $\pm$ .01 \\
banknote & 1.00 $\pm$ .00 & 1.00 $\pm$ .00 & .99 $\pm$ .00 & \cellcolor{custom-grey}1.00 $\pm$ .00 \\
breast cancer & .96 $\pm$ .00 & .97 $\pm$ .01 & .94 $\pm$ .01 & \cellcolor{custom-grey}.95 $\pm$ .02 \\
cars & .82 $\pm$ .01 & .92 $\pm$ .01 & .78 $\pm$ .01 & \cellcolor{custom-grey}.88 $\pm$ .01 \\
contraceptive & .59 $\pm$ .01 & .57 $\pm$ .01 & \cellcolor{custom-grey}.58 $\pm$ .01 & .53 $\pm$ .02 \\
iris & .99 $\pm$ .01 & .99 $\pm$ .01 & .95 $\pm$ .02 & \cellcolor{custom-grey}.96 $\pm$ .02 \\
steel & .68 $\pm$ .01 & .70 $\pm$ .02 & \cellcolor{custom-grey}.68 $\pm$ .01 & .67 $\pm$ .01 \\
students & .58 $\pm$ .02 & .53 $\pm$ .01 & \cellcolor{custom-grey}.45 $\pm$ .01 & .41 $\pm$ .03 \\
\hline
\end{tabular}
\label{tab:performancesVS}
\end{center}
\end{table}

\begin{table*}[t!]
\caption{
Performance of \ac{MoDT} with a \ac{2D} gate.}
\begin{center}
\begin{tabular}{ |r|r|r|R{1.2cm}|R{1.2cm}|R{1.2cm}|r|R{1.7cm}| } 
\cline{2-8}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\ac{MoDT} \ac{2D} d$=$2 e$=$3} & \multicolumn{3}{c|}{\ac{DT}} & \multicolumn{2}{c|}{\ac{RF}} \\
\hline
dataset & training & test & d$=$2 &$d=3$ & $d=4$ & d$=$2 e$=$3 & d$=$*$~$e$=$100  \\
\hline
abalone & .74$\pm$.00 & \cellcolor{custom-grey}.71$\pm$.01 & .67$\pm$.01 & .69$\pm$.01 & .70$\pm$.01 & .67$\pm$.01 & .73$\pm$.01 \\
banknote & 1.00$\pm$.00 & \cellcolor{custom-grey}.99$\pm$.00 & .91$\pm$.02 & .93$\pm$.01 & .95$\pm$.02 & .89$\pm$.04 & .99$\pm$.00 \\
breast & .96$\pm$.00 & \cellcolor{custom-grey}.94$\pm$.01 & .91$\pm$.02 & .92$\pm$.02 & .92$\pm$.02 & .91$\pm$.02 & .94$\pm$.02 \\
cars & .82$\pm$.01 & .78$\pm$.01 & .78$\pm$.02 & .79$\pm$.01 & \cellcolor{custom-grey}.81$\pm$.02 & .71$\pm$.02 & .96$\pm$.01 \\
contraceptive & .59$\pm$.01 & \cellcolor{custom-grey}.58$\pm$.01 & .48$\pm$.02 & .52$\pm$.03 & .55$\pm$.02 & .46$\pm$.04 & .52$\pm$.02 \\
iris & .99$\pm$.01 & \cellcolor{custom-grey}.95$\pm$.02 & .94$\pm$.03 & .94$\pm$.04 & .94$\pm$.03 & .92$\pm$.06 & .95$\pm$.03 \\
steel & .68$\pm$.01 & \cellcolor{custom-grey}.68$\pm$.01 & .53$\pm$.02 & .53$\pm$.02 & .61$\pm$.02 & .53$\pm$.02 & .78$\pm$.02 \\
students & .58$\pm$.02 & .45$\pm$.01 & .48$\pm$.04 &\cellcolor{custom-grey} .51$\pm$.03 & .50$\pm$.04 & .44$\pm$.06 & .49$\pm$.03 \\
\hline
\end{tabular}
\label{tab:performance_2d}
\end{center}
\end{table*}

\begin{table*}[t!]
\caption{Performance of \ac{MoDT} with a \acf{FG}.}
\begin{center}
\begin{tabular}{ |r|r|r|R{1.2cm}|R{1.2cm}|R{1.2cm}|r|R{1.7cm}| } 
\cline{2-8}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\ac{MoDT} FG d$=$2 e$=$3} & \multicolumn{3}{c|}{\ac{DT}} & \multicolumn{2}{c|}{\ac{RF}} \\
\hline
dataset & training & test & d$=$2 &$d=3$ & $d=4$ & d$=$2 e$=$3 & d$=$*$~$e$=$100  \\
\hline
abalone & .75$\pm$.01 & \cellcolor{custom-grey}.73$\pm$.01 & .67$\pm$.01 & .69$\pm$.01 & .71$\pm$.02 & .66$\pm$.01 & .73$\pm$.01 \\
banknote & 1.00$\pm$.00 & \cellcolor{custom-grey}1.00$\pm$.00 & .90$\pm$.02 & .93$\pm$.01 & .96$\pm$.02 & .90$\pm$.04 & .99$\pm$.00 \\
breast & .97$\pm$.01 & \cellcolor{custom-grey}.95$\pm$.02 & .92$\pm$.03 & .92$\pm$.02 & .92$\pm$.02 & .91$\pm$.02 & .94$\pm$.02 \\
cars & .92$\pm$.01 & \cellcolor{custom-grey}.88$\pm$.01 & .78$\pm$.02 & .80$\pm$.02 & .81$\pm$.02 & .71$\pm$.03 & .96$\pm$.01 \\
contraceptive & .57$\pm$.01 & .53$\pm$.02 & .48$\pm$.02 & .52$\pm$.02 & \cellcolor{custom-grey}.55$\pm$.03 & .46$\pm$.04 & .51$\pm$.02 \\
iris & .99$\pm$.01 & \cellcolor{custom-grey}.96$\pm$.02 & .94$\pm$.03 & .95$\pm$.03 & .95$\pm$.03 & .93$\pm$.06 & .95$\pm$.03 \\
steel & .70$\pm$.02 & \cellcolor{custom-grey}.67$\pm$.01 & .53$\pm$.02 & .54$\pm$.02 & .61$\pm$.02 & .53$\pm$.02 & .78$\pm$.02 \\
students & .53$\pm$.01 & .41$\pm$.03 & .48$\pm$.04 & \cellcolor{custom-grey}.51$\pm$.03 & .49$\pm$.04 & .43$\pm$.06 & .48$\pm$.04 \\

\hline
\end{tabular}
\label{tab:performance_full}
\end{center}
\end{table*}


If there is no limit on the size of a tree, the training algorithm might create a large structure that overfits the training data, resulting in great performance on the training data but suboptimal performance on unseen data. Options to limit the creation of new nodes include enforcing a maximum depth or a maximum number of leaves \cite{scikit-learn}.

A problem of DTs is their lack of smoothness in predictions. As the predictions are based on strict splits, a minimal input change in just one of many dimensions can drastically change the output. This is especially problematic when DTs are used for regression problems where one would expect the underlying function to be smooth \cite{Hastie2009}. This becomes particularly notable when a DT has a small number of leaves, as the number of leaves corresponds to the maximum number of distinct values a DT prediction can have. 

%TODO: Graphic?
Furthermore, a common problem of DT training algorithms is the instability of the resulting trees when the training data is modified slightly \cite{Molnar2019}. %Check again change the sentence
Small changes in the training input can lead to very different tree structures regarding the order of the splits, the features included in the splits, and the decision values of the splits. 
This is mainly due to the hierarchical structure of DTs as a change at the top of the tree propagates through all subsequent nodes \cite{Hastie2009}. 
%Maybe Hastie: Linear combination splits, difficulty with additive structure

An advantage of DTs is that they are able to capture interactions between features, i.e., when features are not independent. Due to the hierarchical structure, the method can identify local patterns that are valid for a subset of the training data. DTs implicitly perform a feature selection as not all features are usually included in the final model. This can be an advantage because the user learns which features are probably important, however, also a disadvantage, if features are excluded that the user wanted to assess. Another advantage of DTs is that the training process is usually very fast in comparison to other ML methods such as deep neural networks. 
Arguably, the greatest benefit of DTs is their ability to be understandable for humans. Yet, while small trees are considered to be very interpretable, DTs can quickly become hard to understand if too many nodes are included. Therefore, the complexity of a DT is typically limited when interpretability is desired. An elaboration on what level of complexity is suitable for IML is given in Chapter \ref{ch04}. Further, as the perceived complexity is also largely influenced by the visualization of a DT, various options for the creation of the visualization are discussed as well.

 It is usually not known to which extend such sub populations are present in the input space and how they can be separated. Techniques to explore the presence of sub populations include clustering, mixture models (including MoE), latent class analysis \cite{Vermunt2004} and the tau-path test \cite{Yu2011}.
 
 Firstly, the dimension of model-specificness separates the methods by the criterion of whether they can be used on any underlying ML model, or if they only work with a specific type of model. The former methods are described as model-agnostic and the latter as model-specific \citep{Carvalho2019}. Secondly, it is possible to categorize the methods of IML from a temporal perspective, in relation to the creation of the to-be analyzed ML model.

From the temporal perspective, IML methods that are performed after the creation of the to-be analyzed ML model are captured under the term post-model or \textbf{post-hoc interpretability} \citep{Laugel2019,Lipton2018,Carvalho2019}. These methods are usually---but not necessarily---model-agnostic \citep{Adadi2018}. 

An example of a model-agnostic post-hoc method is the calculation of feature importances by (slowly) changing values of an input data point and observing changes in the output of the model. This and other model-agnostic methods are useable as long as the output of a model, generated for a user-defined input, is receivable. No further knowledge about the underlying ML model is needed.

In contrast, there are IML methods where interpretability is already gained by the time of the creation of the ML model (\textbf{in-model interpretability}). This is the case for intrinsically interpretable models which are per definition always model-specific \citep{Molnar2019}. An example of an intrinsically interpretable method is a (simple) linear regression. The internal coefficients of a linear regression model can be used to understand how the model is solving the task.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/cs_steel_d2_gate.pdf}
    \caption{Gating function.}
    \label{fig:steel_gate_d2}
\end{figure}

\begin{figure*}[ht]
        \centering
        \adjustbox{trim=0cm 2.8cm 0cm 0cm}{%
        \includesvg[inkscapelatex=false, width=400pt]{figures/cs_steel_d2_t1_s.svg}
        }
        \caption{DT for the green region.}
        \label{fig:csdt1}
\end{figure*}

@inproceedings{lime,
author = {Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
title = {"Why Should I Trust You?": Explaining the Predictions of Any Classifier},
year = {2016},
isbn = {9781450342322},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2939672.2939778},
doi = {10.1145/2939672.2939778},
booktitle = {Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
pages = {1135–1144},
numpages = {10},
keywords = {explaining machine learning, interpretability, black box classifier, interpretable machine learning},
location = {San Francisco, California, USA},
series = {KDD '16}
}
@inproceedings{shap,
 author = {Lundberg, Scott M and Lee, Su-In},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {A Unified Approach to Interpreting Model Predictions},
 url = {https://proceedings.neurips.cc/paper/2017/file/8a20a8621978632d76c43dfd28b67767-Paper.pdf},
 volume = {30},
 year = {2017}
}




==> math.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   Identification
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\NeedsTeXFormat{LaTeX2e}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   Preliminary declarations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\RequirePackage{bm} % correct bold symbols, like \bm
\RequirePackage{amsmath}
\RequirePackage{amsfonts}
\RequirePackage{amssymb}
%\RequirePackage{mathrsfs}
%\RequirePackage{dsfont} % double stroke symbols like IR
%\RequirePackage[single]{accents} % own accents 
%\RequirePackage{exscale} % Scaling of Math Symbols?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   Options
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   More declarations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%------------------------------------------------------------
% Mathematical Formulae
%------------------------------------------------------------
\newcommand{\rv}[1]{\ensuremath{{\boldsymbol{#1}}}}
\renewcommand{\vec}[1]{\ensuremath{{\underline{#1}}}}
\newcommand{\rvec}[1]{\ensuremath{{\boldsymbol{\underline{#1}}}}}
\newcommand{\mat}[1]{{\ensuremath{{\mathbf{#1}}}}}

\newcommand{\SquareRoot}[1]{{\mbox{\bfseries\sffamily #1}}}
\newcommand{\intndim}{\ds\int_{-\infty}^\infty \dots \int_{-\infty}^\infty}
\newcommand{\Eye}{\mat{I}}

% operators (in alphabetical order):
\renewcommand{\arg}{\operatorname*{arg}}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\argmin}[1]{\mathop{\mathrm{arg}\; \min_{#1}}}
\newcommand{\argmax}[1]{\mathop{\mathrm{arg}\; \max_{#1}}}
\def\DEF{\triangleq} % definition symbol
\DeclareMathOperator{\col}{col}
\newcommand{\dd}{\operatorname{d}\!}
%\def\d{\ensuremath{\operatorname{d}}} % for \int f(x)\d x or \d y / \d y
%\renewcommand{\d}{\ensuremath{\text{d}}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\MI}{I}
\DeclareMathOperator{\ENT}{H}
\DeclareMathOperator{\Proj}{proj}
\renewcommand{\Pr}{\operatorname{P}} 
\DeclareMathOperator{\rang}{rang}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\jj}{j}% complex unit
\DeclareMathOperator{\rect}{rect}
\def\T{^\mathrm{T}} % transpose
\def\inv{^{-1}} % inverse
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator*{\Var}{Var} 
\renewcommand{\arctan}{\operatorname{arctan}}
\newcommand{\atann}{\operatorname{arctan2}}
%\DeclareMathOperator{\atan}{atan}
\def\atan2{\operatorname{atan2}}
\DeclareMathOperator{\pot}{pot}
\DeclareMathOperator{\sign}{sign}

\newcommand{\FromTo}[2]{$#1 = 1,\, \ldots,\, #2$}
\newcommand{\LMInd}{{\operatorname{LM}}}

%---------------------------------------------------------------------
% Abbreviations
%---------------------------------------------------------------------

\def\({\left(}
\def\){\right)}
\def\[{\left[}
\def\]{\right]}

\newcommand{\ds}{\displaystyle}
\newcommand{\ns}{\textstyle}

\newcommand{\NewB}{\ensuremath{\mathds{R}}}
\newcommand{\NewC}{\ensuremath{\mathds{C}}}
\newcommand{\NewN}{\ensuremath{\mathds{N}}}
\newcommand{\NewQ}{\ensuremath{\mathds{Q}}}
\newcommand{\NewR}{\ensuremath{\mathds{R}}}
\newcommand{\NewZ}{\ensuremath{\mathds{Z}}}
\newcommand{\IR}{\NewR}
\newcommand{\IN}{\NewN}
\newcommand{\IZ}{\NewZ}
\newcommand{\IC}{\NewC}

\newcommand{\Gauss}{{\mathcal{N}}}

\setcounter{MaxMatrixCols}{20} %Fuer ams umgebung


%--------------------------------------------------------------------------
%Einheiten mit korrekten Leerzeichen
%Usage: \Meter{\micro}{10} results $10\mu m$ 
\newcommand{\Meter}[2][]{\unit{#2}#1\meter} 
\newcommand{\Volt}[2][]{\unit{#2}#1\volt} 
\newcommand{\Hertz}[2][]{\unit{#2}#1\hertz} 
\newcommand{\Second}[2][]{\unit{#2}#1\second} 
\newcommand{\Pascal}[2][]{\unit{#2}#1\pascal} 
\newcommand{\Euro}[2][]{\unit{#2}#1\euro}

\newcommand{\nm}[1] {\Meter[\nano]{#1}}
\newcommand{\mum}[1]{\Meter[\micro]{#1}}
\newcommand{\mm}[1] {\Meter[\milli]{#1}}
\newcommand{\cm}[1] {\Meter[\centi]{#1}}
\newcommand{\mV}[1] {\Volt[\milli]{#1}}
\newcommand{\ms}[1] {\Second[\milli]{#1}}
\newcommand{\KHz}[1] {\Hertz[\kilo]{#1}}


%------------------------ Random variables ---------------------------
\def\a{\rv a}
\def\v{\rv v}
\def\w{\rv w}
\def\x{\rv x}
\def\y{\rv y}
\def\z{\rv z}

%---------------------------- Vectors --------------------------------
\def\vdel{\vec \delta}
\def\veta{\vec \eta}
\def\vOmega{\vec \Omega}
\def\vsig{\vec \sigma}
\def\va{\vec a}
\def\vb{\vec b}
\def\vc{\vec c}
\def\vd{\vec d}
\def\ve{\vec e}
\def\vf{\vec f}
\def\vg{\vec g}
\def\vh{\vec h}
\def\vmu{\vec \mu}
\def\vp{\vec p}
\def\vs{\vec s}
\def\vpi{\vec \pi}
\def\vthe{\vec \theta}
\def\vu{\vec u}
\def\vv{\vec v}
\def\vw{\vec w}
\def\vx{\vec x}
\def\vy{\vec y}
\def\vz{\vec z}
\def\vxi{\vec \xi}
\def\vB{\vec B}
\def\vF{\vec F}
\def\vJ{\vec J}
\def\vM{\vec M}
\def\vP{\vec P}
\def\vX{\vec X}

%------------------------- Random vectors ----------------------------
\def\rvn{\rvec n}
\def\rvthe{\rvec \theta}
\def\rvv{\rvec v}
\def\rvw{\rvec w}
\def\rvx{\rvec x}
\def\rvy{\rvec y}
\def\rvz{\rvec z}
\def\rvhz{\rvec{\hat z}}
\def\rvxi{\rvec \xi}
\def\rvX{\rvec X}

%---------------------------- Matrices -------------------------------
\def\A{\mat A}
\def\B{\mat B}
\def\C{\mat C}
\def\D{\mat D}
\def\mE{\mat E}
\def\F{\mat F}
\def\G{\mat G}
\def\H{\mat H}
\def\I{\mat I}
\def\J{\mat J}
\def\K{\mat K}
\def\L{\mat L}
\def\M{\mat M}
\def\P{\mat P}
\def\Q{\mat Q}
\def\R{\mat R}
\def\S{\mat S}
\def\U{\mat U}
\def\V{\mat V}
\def\W{\mat W}
\def\X{\mat X}
% Inverse
\def\iA{\A\inv}
\def\iB{\B\inv}
\def\iC{\C\inv}
\def\iD{\D\inv}
\def\iF{\F\inv}
\def\iM{\M\inv}
\def\iQ{\Q\inv}

%------------------------------ Mean ---------------------------------
\def\ha{\hat a}
\def\hg{\hat g}
\def\hv{\hat v}
\def\hw{\hat w}
\def\hx{\hat x}
\def\hy{\hat y}
\def\hz{\hat z}
\def\hva{\hat{\vec a}}
\def\hvg{\hat{\vec g}}
\def\hvh{\hat{\vec h}}
\def\hvv{\hat{\vec v}}
\def\hvw{\hat{\vec w}}
\def\hvx{\hat{\vec x}}
\def\hvy{\hat{\vec y}}
\def\hvz{\hat{\vec z}}
\def\hvX{\hat{\vec X}}

%------------------------------ Sets ---------------------------------
\def\SA{\mathcal A}
\def\SB{\mathcal B}
\def\SC{\mathcal C}
\def\SD{\mathcal D}
\def\SE{\mathcal E}
\def\SF{\mathcal F}
\def\SG{\mathcal G}
\def\SI{\mathcal I}
\def\SL{\mathcal L}
\def\SM{\mathcal M}
\def\SN{\mathcal N}
\def\SO{\mathcal O}
\def\SP{\mathcal P}
\def\SS{\mathcal S}
\def\ST{\mathcal T}
\def\SU{\mathcal U}
\def\SV{\mathcal V}
\def\SW{\mathcal W}
\def\SX{\mathcal X}
\def\SY{\mathcal Y}
\def\SZ{\mathcal Z}

%------------------------------ Misc ---------------------------------
\def\ii{^{(i)}}
\def\ij{^{(j)}}
